View-Consistent 3D Editing with Gaussian Splatting

The advent of 3D Gaussian Splatting (3DGS) has revolutionized 3D editing, offering efficient, high-fidelity rendering and enabling precise local manipulations. Currently, diffusion-based 2D editing models are harnessed to modify multi-view rendered images, which then guide the editing of 3DGS models. However, this approach faces a critical issue of multi-view inconsistency, where the guidance images exhibit significant discrepancies across views, leading to mode collapse and visual artifacts of 3DGS. To this end, we introduce View-consistent Editing (VcEdit), a novel framework that seamlessly incorporates 3DGS into image editing processes, ensuring multi-view consistency in edited guidance images and effectively mitigating mode collapse issues. VcEdit employs two innovative consistency modules: the Cross-attention Consistency Module and the Editing Consistency Module, both designed to reduce inconsistencies in edited images. By incorporating these consistency modules into an iterative pattern, VcEdit proficiently resolves the issue of multi-view inconsistency, facilitating high-quality 3DGS editing across a diverse range of scenes. Further video results are shown in http://vcedit.github.io.

==> section/intro_backup.tex <==
\section{Introduction}

% 写成我们提的iterative，不要太明显，说清楚为什么iterative有用，注意tone

% 强调“用户提供的gs编辑”就是用户看了第一个gs然后觉得怎么改 —— 谁来重建 —— 图 —— 修改原图，sds再说
% 一句话带过——最近的like xxx 用的完整image editing，发现效果更好 + user friendly
% 1. 点出我们的范式，他好 2. 什么是image-based editing

% 既然修改图就有consistency的问题： however

% 怎么解决consistency的问题，列一些图，不提编辑的名字infedit说sota，发现不consistency —— 提一个effective的概念，按理说整个都要编辑的，但是只有少量的是consistent的编辑

% 这种diverse就会导致“模糊” —— model collapse：几个现象：1.伪影 2.模糊不像 —— figure 2a完成

% 提iterative —— 虽然有些model collapse问题，如果把它当成下一次编辑的基础，可能就成了（其实也不是特别严密）

% 既然iterative，编辑就必须要高效，而且每个iterative必须再加强consistency，如果每一步都能保证成功率更高，下一步收敛更快

% \noindent
% \textbf{1. Intro to Gaussian Splatting, why we edit it?, why first edit image?}

% \denote{point out the task: 3D editing through gaussian splatting, and introduce the importance of it in real world applications.}

% 一开始先点出3d editing，应用
% We consider the editing of 3d vision contents with text instruction. This endeavor hold critical importance in diverse applications, such as development of digital gaming and 3D related design industry.
% % gaussian render快，质量好，方便edit，然后参考gaussian editor的写法
% Recently, Gaussian splatting has emerged as an edit-friendly representation, notable for its rapid processing and superior rendering quality. As an explicit representation, it supports localized operations, making it especially suitable for precise editing and operation of 3D models.
% % 所以使用gaussian做editing是一个比较promising的方向
% Given its characteristics, utilizing Gaussian splatting for 3D editing presents a promising direction in current research.

We consider the problem of text-driven 3D field editing, a task of paramount importance across a variety of industrial applications, such as real-time outfit modifications for 3D digital humans and immersive AR/VR interactive systems. 
Previous 3D field editing~\cite{xx} have predominantly utilized neural radiance fields (NeRF)~\cite{xx}, which equip with high-dimensional multilayer perception (MLP) which intrinsically  entangle shape and apperence. Such computation complexity and lack of precise controllability hinder practical applications, particularly in intricate 3D scene scenarios.

Fortunately, the recent progress in 3D Gaussian Splatting (3DGS)~\cite{xx} emerged as a promising ``Silver Bullet'' for 3D editing, notable for its efficient, high-fidenity rendering, and featuring explicit represenations (3D anisotropic balls) suitable for local manipulation.  
Existing methods~\cite{xx} leverage the off-the-sheff 2D editing models~\cite{xx} to guide the optimization of 3DGS. 
This pattern holds plausible editing effects and facilitates user-friendly interaction.
Specifically, it renders source 3DGS into multi-view 2D images, manipulates them via 2D editing models using text prompts, and then employs these adjusted images to fine-tune the original 3DGS. 
% \textcolor{green}{It allows users to provide their desired edited images and customize the editing process.}
% \textcolor{green}{Beyond its high-quality editing effects, such image-guided editing also facilitates user-friendly interaction, allowing users to provide their desired edited images and customize the editing process.}


% As an explicit representation, it supports localized operations, making it especially suitable for precise editing and operation of 3D models. Given its characteristics, utilizing Gaussian splatting for 3D editing presents a promising direction in current research.

% \noindent
% \textbf{2. Why image-based editing?}

% 强调“用户提供的gs编辑”就是用户看了第一个gs然后觉得怎么改 —— 谁来重建 —— 图 —— 修改原图，sds再说
% 一句话带过——最近的like xxx 用的完整image editing，发现效果更好 + user friendly: This approach allows us to complete preliminary data modifications before fine-tuning NeRF, as well as enabling users to determine 3D content by selecting the editing results from key 2D views.
% 1. 点出我们的范式，他好 2. 什么是image-based editing

% Current approaches~\cite{xx} to Gaussian Splatting Editing leverage an image-editing guidance. 
% % Specifically, it applies image editing models' output as training images to refine the Gaussian.
% Specifically, the process begins by rendering the source Gaussian into 2D images views, which are then edited through Stable Diffusion model. Subsequently, it applies the edited images as training data to adjust the Gaussian.
% Beyond its high-quality editing effects, this approach also facilitates user-friendly interaction, allowing users to provide their desired edited images and customize the editing process.


% achieving excellent editing effects while maintaining user-friendliness.
% This approach allows us to complete preliminary data modifications before fine-tuning NeRF, as well asenabling users to determine 3D content by selecting the editing results from key 2D views.
% \noindent
% \textbf{3. Cross-View Inconsistency Issue: why iterative? why consistency control?}

% 既然修改图就有consistency的问题: however
% However, this image-editing guidance has a view inconsistency challenge that cannot be ignored. 
% % figure 2a
% In Figure 2a, we showcase the independently edited outcomes achieved through a state-of-the-art image editing model. 
% We note considerable inconsistencies across the edits of different views. 
% This issue arises because each view is processed separately by the Stable Diffusion model, lacking awareness of other views.
% % When applying such inconsistent views as guidance, the 3D Gaussian model might face the guidance where only few of views are consistent, while others conflict with each other.
% % Unfortunately, the explicit nature of Gaussian Splatting makes it exhibits heightened sensitivity to guidance that lacks view-consistency. 
% When utilizing these inconsistently edited images as guidance, the 3D Gaussian model may encounter the trouble where only a few training images are consistent, while the others present conflicting information. 
% Unfortunately, due to the explicit nature of Gaussian Splatting, it demonstrates an heightened sensitivity to guidance that lacks view-consistency.
% Consequently, directly using image-editing guidance in training may result in a phenomenon called mode collapse, showcased as the learned Gaussian exhibiting ambiguity between the source and target, along with flickering artifacts observable from certain perspectives.

% figure 2a
% As shown in Figure 2a, the sperately edited images through a state-of-the-art 2D editing model~\cite{xx}, showcase considerable view inconsistencies. 
% This issue arises because each view is processed separately by the 2D editing model, lacking awareness of other views.
% When utilizing these inconsistently edited images as guidance, the 3D Gaussian model may encounter the trouble where only a few training images are consistent, while the others present conflicting information. 
% Unfortunately, due to the explicit nature of Gaussian Splatting, it demonstrates an heightened sensitivity to guidance that lacks view-consistency.
% Consequently, directly using image-editing guidance in training may result in a phenomenon called mode collapse, showcased as the learned Gaussian exhibiting ambiguity between the source and target, along with flickering artifacts observable from certain perspectives.

%承接关系，2D inconsistent 因为不是3D aware；导致的后果是gassuain mode collpse，这会由于gassian的特性带来异常的editing challenge。
However, image-guided 3DGS editing has well-documented multi-view inconsistency that cannot be ignored.
Figure~\ref{xx} vividly illustrates that images edited separately using a state-of-the-art 2D editing model~\cite{xx} exhibit significant view inconsistencies --- the four views of a man are edited to different style of clowns.
We believe such problem stems from the lack of 3D awareness in 2D editing models, that is, they inherently process each view in isolation.
When these highly diverse edited images are leveraged as guidance, the 3DGS model struggles with the issue that only a few training images are coherent, whereas the majority display conflicting information.
Unfortunately, the explicitness and inherent densification pattern of 3DGS makes it especially vulnerable to high variance of image guidance~\cite{xx}.
Consequently, directly employing multi-view image guidance can lead to mode collapse, characterized by the learned 3DGS's ambiguity between the source and target, as well as the flickering artifacts in Figure~\ref{xx}.


% 提一个effective的概念，按理说整个都要编辑的，但是只有少量的是真正有用的，consistent的编辑（hw提的，但这里不知道怎么写合适了）
% \reddenote{In other words, the editing process is ineffective, since only few or even none views are consistently edited.}
% 这种diverse就会导致“模糊” —— model collapse：几个现象：1.伪影 flickering artifacts 2.模糊不像 ambiguity —— figure 2a讲完了
% When applying such inconsistent views as guidance, the 3D Gaussian model attempts to accommodate the varied modifications of each view during its training phase. 
% Given the explicit nature of Gaussian Splatting, it exhibits heightened sensitivity to guidance that lacks view-consistency.
% Therefore, the diversity among the inconsistent views can lead to a phenomenon known as mode collapse, presenting as the learned Gaussian exhibiting ambiguity between the source and target, coupled with flickering artifacts when viewed from certain perspectives.

% 提iterative —— 虽然有些model collapse问题，如果把它当成下一次编辑的基础，可能就成了（其实也不是特别严密）
% To address the issue of inconsistency, we introduced the \textit{View-Consistent Editor (VCEditor)} taylored for Gaussian Splatting. 
% Parallel to previous works \cite{xx}, we conjecture that an iterative editing pipeline — editing views, training the Gaussian with these views, and repeating this process — is beneficial to resolve the inconsistencies.
% The rationale behind is that each iteration builds upon the outputs of the previous one, allowing views that were edited inconsistently in one iteration to be improved in subsequent iterations. 
% As a result, the proportion of accurately edited views escalates with each iteration, facilitating a progressive refinement of the Gaussian with ongoing process.
% Due to the reliance on multiple cycles for each view, the processing speed of the image editing model becomes a critical requirement in the iterative pipeline.
% Therefore, in \textit{VCEditor}, we employs InfEdit \cite{xx}, a state-of-the-art image editing model with rapid speed and high quality. It gets rid of time-cosing DDIM-inversion stage for faster processing speed.
% In each iteration, our approach edits all views simultaneously, facilitating the cross-view control on editing consistency.
% We illustrate our iterative process in Figure 2b, where the edited gaussian is iteratively guided to a consistent style that aligns with the desired target.

%The crux for ... is to make xxx.
% To address the multi-view inconsistency issues in image guidance, we introduced the \textit{View-Consistent Editor (VCEditor)} specifically designed for 3DGS. Our key insights includes iterative pattern and consistency control design.
% Parallel to prior research \cite{xx}, we conjecture that an iterative pattern --- editing views, training the 3DGS with these views, and repeating this process --- is beneficial to resolve the inconsistencies.
% The iterative process inherently builds on the outputs of previous cycles, allowing for the correction of initially inconsistent views in later iterations and promoting the continuous improvement of 3DGS.
% We illustrate the iterative pattern in Figure 2b, where the 3DGS is progressively guided to a consistent style that aligns with the desired target.
% Given the iterative pattern's demands on the 2D editing model's speed, \textit{VCEditor} employs InfEdit \cite{xx}, a leading-edge image editing model known for its speed and quality, which eliminates the time-consuming DDIM-inversion stage for efficiency.

% Therefore, the crux lies in \textbf{enhancing the multi-view consistency of image guidances}.
% To this end, we introduce \textit{View-Consistent Editor (VCEditor)} specifically designed for 3DGS. 
% Our insights includes iterative pattern and consistency control design.
% Parallel to prior work \cite{xx}, we conjecture the iterative pattern --- editing views, training the 3DGS, and repeating --- contributes to rectify the inconsistency. 
% It allows for the correction of initially inconsistent views in later iterations and continualy refine the 3DGS.
% As shown in Figure 2b, the 3DGS of a \textit{man} is iteratively guided to a consistent style that aligns with the desired \textit{clown} target.
% To accommodate the iterative demand for speed, VCEditor integrates InfEdit \cite{xx}, a fast, high-quality image editing model that bypasses the time-consuming DDIM-inversion phase.

Thus, the crux lies in enhancing the multi-view consistency of image guidance.
To this end, we propose \textit{View-Consistent Editor (VCEditor)}, an efficient and controllable 3DGS editing framework with \textit{iterative pattern} and \textit{multi-view consistency control mechanism}.
% Our insights includes iterative pattern and consistency control design.
Parallel to prior work \cite{xx}, we conjecture the iterative pattern --- \textcolor{green}{editing views, training the 3DGS, and repeating} --- contributes to rectify the inconsistency since it allows for the correction of initially inconsistent views in later iterations and continuously refines the 3DGS \textcolor{blue}{[fostering a mutual cycle of xx]}.
As shown in Figure 2b, the 3DGS of a ``man'' is iteratively guided to a consistent style that aligns with the desired ``clown'' target.
To meet the demands for rapid iteration, VCEditor integrates InfEdit \cite{xx}, a swift, high-quality image editing model that bypasses the lengthy DDIM-inversion~\cite{xx} phase.

Building upon the iterative pattern, our key insight centers on consolidating multi-view edited images \textit{within} iteration, thereby enabling superior quality edits.
Harnessing 3DGS's explicit representation and fast rendering capability, we introduce a multi-view \textit{Consistency Control Framework (CCF)} for each editing iteration.
% By minimizing the multi-view editing discrepancy, our approach effectively prevents the edited views from diverging.
As depicted in Figure 2b, our \textit{CCF} minimize the multi-view editing discrepancy utilizing two main elements:
\begin{itemize}
\setlength{\itemsep}{2pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
% \vspace{-1em}
% \item A \textit{Prediction Consistency Control} mechanism is utilized for harmonizing divergent editing predictions by fine-tuning a source-cloned 3DGS with original multi-view predictions and rendering the adjusted 3DGS across views for unified outcomes. 

\item We deploy a \textit{Prediction Consistency Control} mechanism. It harmonizes the divergent editing predictions by utilizing the inherent slight calibration capability of 3DGS~\cite{xx}.
Specifically, we use the original predictions to fine-tune a source-cloned 3DGS with original predictions, subsequently rendering it across views to produce unified predictions. The mechanism relies on 3DGS's fast training and rendering,
% calibration 能力 - harmony
% harness the fast training speed of 3DGS

\item The \textit{Cross-Attention Consistency Control} integrates into each U-Net layer within InfEdit.
Using 3DGS's explicit coordinates, it first back-projects the attention maps to 3D space to build an averaged 3D map, and then render it back to obtain 3D-awared attention maps.
The mechanism calibrates the model's attentive regions across all views, substantially enhancing the prediction and blending steps of InfEdit.
\end{itemize}
% \vspace{-1em}

% In summary, VCEditor excels in 3DGS editing by ensuring multi-view consistent image guidance, leading to superior editing quality as demonstrated by extensive experiments (Section~\ref{xx}). \textcolor{green}{Surprisingly, it is observed that most samples achieve high-quality outcomes with just two editing iterations.}

As illustrated in Figure~\ref{fig:1}, by incorporating the xxx and xxx, VCEditor significantly enhances multi-view consistent image guidance, leading to superior editing quality. 
We demonstrate the superiority of VCEditor on xxx. 
We conduct comprehensive evaluations of VCEditor across various real-world scenes, including objects, human faces, and outdoor scenes.
Both qualitative and quantitative comparisons clearly show that VCEditor can xxx, continually outperforming other state-of-the-art methods. 
Our contributions can be summarized in three aspects:
\begin{itemize}
\setlength{\itemsep}{2pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
% \vspace{-1em}

\item We propose an effective \textit{Consistency Control Framework} that harmonizes the inconsistent multi-view image guidances.
\item Based on our consistency controlling design, we construct an effective iterative pipeline that offers high-quality 3DGS editing.
\item We pioneeringly offer a paradigm that integrates 3DGS with multi-view consistency design, inspiring future efforts towards further exploration.
\end{itemize}

% make the mask 3d-aware, unifying the 3d location which the model cares, guide the prediction and postprocessing in InfEdit.

% First, we deploy a \textit{Prediction Consistency Control} mechanism to consolidate the inconsistent editing predictions.
% Starting by collecting the original multi-view predictions, we use them to fine-tune a 3DGS cloned from the source. 
% Then, we render the fine-tuned 3DGS onto each view to generate consolidated predictions.
% Secondly, we design another \textit{Cross-Attention Consistency Control} to each U-Net layer in InfEdit. 
% Utilizing the 3D coordinates in 3DGS explicit representation, we employ back-projection and rendering to consolidate multi-view cross-attention maps and diminish their discrepancy.



% Parallel to prior work \cite{xx}, we conjecture the iterative pattern --- editing views, training the 3DGS, and repeating --- contributes to rectify the inconsistency. 
% It allows for the correction of initially inconsistent views in later iterations and continualy refine the 3DGS.
% As shown in Figure 2b, the 3DGS of a \textit{man} is iteratively guided to a consistent style that aligns with the desired \textit{clown} target.
% To accommodate the iterative demand for speed, VCEditor integrates InfEdit \cite{xx}, a fast, high-quality image editing model that bypasses the time-consuming DDIM-inversion phase.


% Built upon the iterative pattern, our primary insight focuses on enhancing multi-view consistency in each iteration, thereby achieveing superior editing quality with fewer iterations.
% In \textit{VCEditor}, one iteration incorporates an InfEdit pass comprising sequential image editing timesteps (timesteps), with each one enhancing the editing prediction from its predecessor, progressively moving the edited image towards the target.
% During each timestep, we introduced a multi-view \textit{Consistency Control Framework (CCF)} that edits all views concurrently. 
% Utilizing the explicit representation and real-time rendering features of 3DGS, our method minimizes the multi-view editing variances, preventing the edited views from diverging as the denoising step progresses. 
% In Figure 2b, we illustrate that after applying \textit{CCF} in a single iteration, the consistency of multi-view edited images is markedly enhanced.
% Our \textit{CCF} includes two crucial components:

% First, by utilizing the rapid training and rendering capabilities of 3DGS, we deploy a \textit{Prediction Consistency Control} mechanism to consolidate the predictions of each timestep.
% Starting with collecting the original multi-view predictions, we use them to fine-tune a 3DGS cloned from the source. 
% Since the predictions at each timestep change minimally from their inputs, the inconsistency between multi-view predictions is reduced, thus averting the risk of mode collapse during fine-tuning.
% Subsequently, we render the fine-tuned 3DGS onto each view to generate consolidated predictions, forwarding them to the next timestep.

% We develop another consistency control to consolidate multi-view cross-attention maps of each layer in U-Net. 
% Utilizing the 3D coordinates in 3DGS explicit representation, we back-project the multi-view cross-attention maps into 3D space and calculate the mean value for each 3D location.
% Then we render the 3D map back to all views to replace the original attention maps. 
% Our experiments demonstrate that the cross-attention control mechanism provides an additional support for view consistency.

% Built upon the iterative pattern, our primary insight focuses on enhancing multi-view consistency in each iteration, thereby achieveing superior editing quality with fewer iterations.
% We introduced a multi-view \textit{Consistency Control Framework (CCF)} that edits all views concurrently. 
% Utilizing the explicit representation and real-time rendering features of 3DGS, our method minimizes the multi-view editing variances, preventing the edited views from diverging.
% Our \textit{CCF} includes two crucial components:

% First, we deploy a \textit{Prediction Consistency Control} mechanism to consolidate the inconsistent editing predictions.
% Starting by collecting the original multi-view predictions, we use them to fine-tune a 3DGS cloned from the source. 
% Then, we render the fine-tuned 3DGS onto each view to generate consolidated predictions.
% Since the predictions at each timestep change minimally from their inputs, the inconsistency between multi-view predictions is reduced, thus averting the risk of mode collapse during fine-tuning.
% Secondly, we design another \textit{Cross-Attention Consistency Control} to each U-Net layer in InfEdit. 
% Utilizing the 3D coordinates in 3DGS explicit representation, we employ back-projection and rendering to consolidate multi-view cross-attention maps and diminish their discrepancy.
% % Utilizing the 3D coordinates in 3DGS explicit representation, we back-project the multi-view cross-attention maps into 3D space and calculate the mean value for each 3D location.
% % Then we render the 3D map back to all views to replace the original attention maps. 
% Our experiments demonstrate that the cross-attention control mechanism provides an additional support for view consistency.
% In Figure 2b, we illustrate that after applying \textit{CCF} in a single iteration, the consistency of multi-view edited images is markedly enhanced.


% 这里把我们的less iteration的contribution提出来！我们惊喜地发现我们的方法在简单的1-2个iteration就能取得很好的效果

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.99\linewidth]{latex/figure/figure2.pdf}
% \caption{Illustration of different iterations' rendered view of GaussianEditor, each iteration includes an image editing process. As the number of iterations increases, the level of editing continuously improve.}
% \label{fig:iterative}
% \end{figure}

==> section/method_backup.tex <==
\section{Methods}
% 3.4：建议把所有的定义全部放在preliminary里面讲清楚，overview不需要单独成section，只需要在methods最前面有一段总起的进行说明；4.2和4.3用词要严谨，科学，规范，时态问题，input和output，承上启下，上下文逻辑一句一句理一遍。能用一句话讲清楚的绝不用2句话，要把每一段表达什么意思都先列出来；最后overall的loss是什么都没有看到；对于iteration的定义是不是在iterative pattern里进行说明就好，前面默认是一个iteration？？


% 4
% 我们通过diffusion model来进行image-based editing，并通过我们提出的A和B来改善传统image-based editing的consistency问题。具体来说，我们在Sec4.1介绍如何xxxx，Sec4.2介绍如何通过attention consistency改善xx 

% 4.1
% 1.讲framework的图。

% Given a xx，我们先利用pretrained diffusion model来生成initial prediction。Specifically，讲time step，add noise，denoise等。To further 保证 xx（讲attention consistency的作用），我们提出这个，然后写一句话总结这个方法。Details are in Sec4.2

% 得到了intial prediction之后，我们希望能够进一步提高这些guidance的consistency，并提出了prediction consistency control。Specifically，一句话总结。Details are in xx。

% 最后，这一段话简述一下利用生成好的consistent的guidance进行iterative的edit，不提local blend

% 4.2 Attention Consistency Control
% %简述这个模块的目的，两个。1. 改善unet的output的consistency。2.提取出的attention map用于保留未被edit的细节。（high-level的讲目的，不提任何实现）
% 简述这个模块的目的——改善unet的output的consistency。不提local blend

% 陈述问题起手，现有的2D diffusion model生成的图片缺乏multiview consistency，我们argue这是因为多次生成的unet之间信息没有交互。为了解决这个，我们将xxx（讲怎么fusion这些attention map）。通过用我们这种fused attention代替unet原有的vanilla attention，我们给予了生成的图片一定的consistency，如figxx。
% （这段话写的详细一点，不然没写的）

% 4.3 Predicition Consistency Control
% 通过4.2介绍的attention control，unet生成的图已经具有一定的consistency，但其精确性不足以直接用于update 3DGS（cue图来illustrate，或者exp里面的ablation）。( Inspired by xx，感觉有点像sds的原理，通过用图片来训练一个物理建模来增强consistency，没有inspired的话可以不写)，我们提出可以先将image guidance蒸馏进一个具有物理建模和consistency的intermediate model，并通过该model产生精确的consistent guidance。本文中我们直接通过fine-tune source 3DGS来完成这一步骤。

% Specifically，讲具体实现

% 特别的，为了保留未被edit的细节，我们follow xx 使用了local blend的方法，列公式

% 其中xx是sec4.2中的fused attention，xxfine-tuned的3DGSrender的图片

% Given a source 3DGS, denoted by $\gsrc$, and a user-specified target prompt $\y$, our goal is to transform $\gsrc$ into an edited version $\gedt$ that aligns with $\y$. The main challenge lies in preserving $\gsrc$'s essential content while achieving high fidelity in the edits as per $\y$.

% Leveraging this image-guided editing pipeline, we characterize each transition of ``$\gsrc \rightarrow \Isrc \rightarrow \Iedt \rightarrow \gedt$'' as an iteration. 
% \textcolor{red}{one sentence, how we use infedit in image editing, introduce t 4.1}
% Given a source 3DGS model $\gsrc$, our VCEditor finetunes $\gsrc$ towards an edit instruction $\y$ into an edited version $\gedt$.

% Our VCEditor utilizes the image-guided 3DGS editing pipeline outlined in Sec.~\ref{3dgs editing}, aiming to solve the mode collapse issue brought by the multi-view inconsistency in $\Iedt+$.
% In Sec.~\ref{sec:imgedit}, we detail the process in VCEditor of editing rendered images, denoted as $\Isrc$, to produce $\Iedt$.
% In the image editing process, we introduce two multi-view consistency control mechanisms leveraging 3DGS's explicit representation and fast rendering capability (illustrated in orange color in Fig.~\ref{fig:method}):
% (1) The \textbf{Prediction Consistency Control} mechanism that directly calibrates the multi-view editing predictions to generate consistent predictions (Sec.~\ref{sec:pcc}).
% (2) The \textbf{Cross-Attention Consistency Control} mechanism that consolidates multi-view cross-attention maps to consistent maps(Sec.~\ref{sec:acc}).
% Finally, we extend our framework to an \textbf{iterative pattern} (Sec.~\ref{sec:iter}), facilitating a mutual enhancement of $\Iedt$ and $\gedt$ against the multi-view inconsistency issue.

Leveraging the Diffusion Model, our VCEditor conducts the image-guided 3DGS editing detailed in Sec.~\ref{3dgs editing}, where we 
propose two consistency control mechanisms to solve the multi-view inconsistency issue in the original image-guided editing.
Concretely, in Sec.~\ref{sec:imgedit}, we outline the editing process of rendered images in VCEditor. 
In Sec.~\ref{sec:acc}, we propose the \textbf{Cross-Attention Consistency Control} mechanism to alleviate the multi-view editing variance by enhancing the attention consistency.
In Sec.~\ref{sec:pcc}, we introduce the \textbf{Prediction Consistency Control} mechanism which directly calibrates the multi-view editing predictions to generate consistent predictions.
Finally, in Sec.~\ref{sec:iter}, we extend our framework to an \textbf{iterative pattern}, facilitating a mutual enhancement of $\Iedt$ and $\gedt$ against the multi-view inconsistency issue.

\textcolor{blue}{need to refer 3DGS like: leveraging 3DGS's explicit representation and fast rendering capability?}

\subsection{Rendered Images Editing}
\label{sec:imgedit}
% \textcolor{red}{don't mention why.}

Given a set of multi-view rendered images, $\Isrc$, we first utilize the pre-trained Diffusion Model to generate the initial predictions.
Specifically, in the Diffusion Model, an image editing process comprises a sequence of descending diffusion timesteps $t$, ranging from $T$ to $1$. 
In each timestep $t$, the multi-view images are first encoded as source latents, denoted as $\zs$. Then, a step-related noise $\eps_t$ is added to $\zs_t$, represented by:
\begin{equation}
    z_t = \sqrt{\alpha_t}\zs + \sqrt{1 - \alpha_t} \eps, \: \eps \sim \mathcal{N}(\mathbf{0}, \mathbf{I})
\end{equation}
The noisy latents $z_t$ are then processed by a U-Net, which predicts the conditional noises, represented as $\eps_\theta(z_t, \y)$.
The initial predictions are obtained by subtracting the conditional noises, represented as:
\begin{equation}
    
\end{equation}
, which serve as the edited latents.


\textcolor{red}{we utilize infedit xxx}
Fig.~\ref{fig:method} illustrates our framework \textit{within} an iteration: 
After rendering $\gsrc$, the image editing process takes as input all-views source images $\Isrc$. \textcolor{blue}{The $\Isrc$ are first encoded to a set of multi-view source latents, denoted as $\zs_{T}=\enc(\Isrc)$. TODO: Also add it in figure} 
Inheriting from InfEdit, an image editing process within VCEditor comprises a sequence of descending diffusion timesteps $t$, ranging from $T$ to $1$. 
\textcolor{blue}{Beginning with $t=T$, each timestep $t$ produces a set of edited latents based on its multi-view input source latents, $\zs_t$. The outputs are subsequently forwarded to the next timestep as input, indicated as $t-1$.}
Each step incrementally enhances the editing predictions over its predecessor, thereby progressively transforming the edited images to more closely match the target. At the last timestep $t=1$, the editing latents are decoded to generate $\Iedt$, represented as $\Iedt = \dec(\ze_1)$.

\textcolor{red}{from 4.2}
As depicted in Fig.~\ref{fig:method}, in the start of each timestep, a step-related noise $\epsilon_t$ is added to the multi-view source latents $\zs_t$. 
These noisy latents are then processed by a U-Net, which predicts the conditional noises, represented as $\bar{\epsilon_t} = \epsilon_\theta(\zs_t, t, \y)$. These predicted noises are then subtracted from the noisy latents. 
Utilizing the text prompts $\y$, this process of adding noise and subsequent denoising transforms $\zs_t$ into multi-view edited latents, $\ze_t = \zs_t + \epsilon_t - \bar{\epsilon}_t$, serving as the editing predictions.
\textcolor{red}{detailed in 4.2}

Building on InfEdit's approach, we enhance each timestep $t$ with a Local Blend operation to better preserve the background information in $\Isrc$.
This method heavily relies on the cross-attention maps from each layer, where pixels are closely aligned with the words describing them. 
% For example, in editing transitions from "man" to "clown", pixels with higher cross-attention weights towards "clown" are more likely to be a part of clown, while the lower weights indicating background that necessitating preservation.
\textcolor{red}{cannot use 3-4 lines for justification. if necessary, use a footnote}
For instance, during editing transitions from "man" to "clown," pixels that have higher cross-attention weights towards "clown" are more likely to be part of the clown, whereas pixels with lower weights are indicative of unedited areas that require preservation.
Thus, given the cross-attention maps $\m$, the source latents $\zs_t$, and the consistent latents $\zc_t$ produced in Sec.~\ref{sec:pcc}, the blending is conducted by:
\begin{equation}
\zb_t = \m * \zc_t  + (1 - \m) * \zs_t
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{latex/figure/figure4.pdf}
\caption{1. add text in PCC. 2. use inverse-color maps 3.refine arrows
4. next iteration 5. change variable name according to 4.1}
\label{fig:method}
\end{figure}


\subsection{Cross-Attention Consistency Control}
\label{sec:acc}
% UNet怎么操作的，camap是什么，意味着什么

During each timestep $t$ of the multi-view image editing process, the U-Net acts as a conditional noise predictor that shapes the edited latents, as illustrated in Fig.~\ref{fig:method}. 
Each U-Net layer incorporates a cross-attention block, where a set of cross-attention maps $\m$ dictate the pixel-to-text token focus to enable interaction between the images and user's prompt, playing a pivotal role in the editing.
% enhancing the interaction between pixel spatial structures and prompt words.
% Within these blocks, the cross-attention maps $\m$ dictate the pixel-to-text token focus, playing a pivotal role in the editing predictions.

\textcolor{blue}{However, these multi-view's cross-attention maps are not consistent due to the independent processing of each view's image.
For instance, regarding the word "clown," a cross-attention map might highlight the left eye in one view and the right eye in another, leading to the same prompt word focusing on mismatched regions across views. This results in inconsistent edits and blending.}

\textcolor{red}{write as a justification, one short sentence for challenge}

Therefore, to unifys the model's attentive region across different view given each word in prompt, in VCEditor, we have developed a mechanism to unify the multi-view cross-attention maps, which we designate as \textbf{Cross-Attention Consistency Control}.
% Therefore, in VCEditor, we have developed a mechanism to unify multi-view cross-attention maps, with the process depicted in Fig.~\ref{fig:method}.


% For example, towards the word "clown", the cross-attention map in one view may assign higher value on the left eye, while other views assigning higher value on the right eye.
% Consequently, a same word in prompt may attends to incoherent regions in different views, leading to inconsistent edited latents and blending.
% however，due to the independent processing of xxx, ca map本身是不consistent的，意味着不同视角的图片中模型的关注区域不coherent。lead to potential inconsistency in predictions and local blend.
% 就该一样——因此我们对ca做了操作

With the process depicted in Fig.~\ref{fig:method}, we project $\gsrc$ onto a 2D plane using the camera matrix of any given view. Building on this foundation, we employ inverse-rendering to map the 2D cross-attention maps $\m_v$ back onto the 3D Gaussians within $\gsrc$.
% Specifically, in each layer, we collect the cross-attention maps of all views, denoted as $\m_v, v \in \Vs$, after they are computed. 
% Utilizing the explicit representation of 3DGS, we build a 3D maps, $\mm$, based on the 2D attention maps. 
% Firstly, we take the $\gsrc$, following the rendering function in Sec.~\ref{}, the $\gsrc$ can be projected to 2D plane given an arbitrary view's camera matrix.
% Based on that, we here implement a inverse-rendering that projects the 2D cross-attention map $\m_v$ to 3D Gaussians in $\gsrc$. 
% Specifically, inspired by the implementation in \cite{}, for the $j$-th Gaussian in $\gsrc$, we maintain a weight along with a counter. 
% Towards the view $v$, the weight for the $j-$th Gaussian is computed as:
% \begin{equation}
%     w_{j, v} = \sum_{\textbf{p}} o_j(\mathbf{p}) \cdot T_{j, v}(\mathbf{p}) \cdot \m_{v, \mathbf{p}}
% \end{equation}
% where $\mathbf{p}$ denotes each pixels in the cross-attention map of $v$. After computing weights for all views, we obtain the 3D maps by average:
Specifically, inspired by the implementation in \cite{}, for the $j$-th Gaussian in $\gsrc$, its value in the 3D map $\mm_j$ is computed as: 
\begin{equation}
    \mm_j = \frac{1}{C_j}\sum_{v \in V} \sum_{\textbf{p}} o_j(\mathbf{p}) \cdot T_{j, v}(\mathbf{p}) \cdot \m_{v, \mathbf{p}}
\end{equation}
where $\mathbf{p}$ is a pixel in a 2D attention map, while $o_i(\mathbf{p})$, $T_{j, v}(\mathbf{p})$, $\m_{v, \mathbf{p}}$ denoting the opacity, transmittance, and cross-attention weight of pixel $\mathbf{p}$. The $C_j$ is the count indicating the total number of values that assigned to $j$ by $\m_{v, \mathbf{p}}$ across all $p$ and $v$.
After creating the 3D map, where each Gaussian is assigned a cross-attention value corresponding to each word in the prompt, we render this 3D map back to 2D, resulting in unified cross-attention maps, $\m^{con}$.

By replacing the original $\m$ with $\m^{con}$, this mechanism unifys the model's attentive region across different view towards each word in the prompt, which facilitates the model to produce more coherent edited latents. 
% Besides, $\m^{con}$ also contributes to a consistent foreground-background recognition in the local blending module. In Sec.~\ref{}, our experiments demonstrate that the cross-attention control mechanism provides an additional support for view consistency.
Furthermore, $\m^{con}$ aids in achieving consistent edited-region recognition within the local blending module. Our experiments, detailed in Sec.~\ref{}, validate that this cross-attention control mechanism significantly bolsters view consistency.

% \begin{align*}
%     &\mathbb{I}(j, v, h, w) = 
%     \begin{cases} 
%     {1}, & \:\text{if } g_v(\gsrc_j) = (h, w) \\
%     {0}, & \:\text{if } g_v(\gsrc_j) \neq (h, w)
%     \end{cases}, \:
%     \: v \in \Vs,\: h \in \left[0, H\right], \: w \in \left[0, W\right] \notag \\
%     &\mm_j = \frac{1}{\sum_{v, h, w} \mathbb{I}(j, v, h, w)} \cdot \sum_{v, h, w} \m_v(h, w) \cdot \mathbb{I}(j, v, h, w)
% \end{align*}

% collect
% 投影矩阵，投影，平均
% rendered back，norm处理

% 效果

% a random noise $\epsilon \in \mathcal{N}(0, 1)$ is added to the multi-view source latents $\zs_t$. Then the noisy latents are passed into a U-Net to predicts an conditional noise, denoted as $\epsilon_\theta(\zs_t, t, )$


\textcolor{red}{dont shout out 3DGS too many times, like "rapid speed"...}
\textcolor{red}{too long}

\textcolor{red}{
1. first sentence directly
2. be concrete in justification
3. decouple the justification and processing, can be both front and behind(if not simple)
4. be concrete in language
}

\textcolor{red}{better not propose a challenge, use 1 sentence to describe the problem.}

\textcolor{red}{remove all above, write like: we employe a xxx to address xxx problem.}

\textcolor{red}{put the ``minimal" changes to the front}

\textcolor{red}{1 sentence or none sentence for problem definition or concrete why we use this module (why it works), we employ xxx , then how we do it, at last why it works}


\subsection{Prediction Consistency Control}
\label{sec:pcc}

% 先讲每个timestep干了啥，输入输出讲明白， cross attn map先不提更新的事情，一直讲到edited latents
% unet和加减噪声过程先不拆开讲，4.3用到再说
% As depicted in Fig.~\ref{fig:method}, after rendering $\gsrc$, the image editing process takes the all-views source images $\Isrc$ as input. 
% \textcolor{blue}{The $\Isrc$ are first encoded to source latents, denoted as $\zs_T$. TODO: Also add it in figure} 
% Then starts from $t=T$, the editing processing starts to cycle the timesteps. After each timestep is finished, the $t$ decrease to $t-1$ and starts a new cycle.

% However, due to each view's edited latent being processed independently, multi-view inconsistency arises in $\ze_t$. In particular, the latent of each view, $\ze_{t, v}$ for $v \in \Vs$, exhibits editing content that is not coherent with the latents from other views.

Our observations indicate that 3DGS possesses a limited capacity to rectify inconsistencies across views when variances in multi-view editing are slight.
Thus, to address the multi-view inconsistency in the edited latents, $\ze$, we suggest employing a 3DGS to calibrate the incoherently edited content across views, generating a new set of consistent latents, denoted as $\zc$. We refer to this calibration process as the \textbf{Prediction Consistency Control} mechanism.

The procedure of this mechanism is illustrated in Fig.~\ref{fig:method}. Specifically, we first decode the multi-view latents $\ze_t$ into images, which are subsequently employed to refine a 3DGS cloned from $\gsrc$:
\begin{equation}
\gft = \: \underset{\G}{\mathrm{argmin}} \: \sum_{v \in \Vs}{ L_{sim}(\mathcal{R}(\G, v),\: \dec(\ze_{t, v})) }
\end{equation}
After the rapid fine-tuning process, we render $\gft$ back onto each viewpoint $v \in \Vs$, yielding a collection of rendered images. Thanks to the calibration capability of 3DGS, these images exhibit significantly reduced incoherence.
Finally, the images are encoded back to obtain the consistent latents, $\zc_t$, which serves as the input of the local blend module. 

Utilizing the rapid training and rendering capabilities of 3DGS, we conduct this fine-tuning and rendering process at each timestep.
% 我们操作的目的，效果——去除了什么什么
% Following the fine-tuning and rendering processes, the latents $\zc_t$ at each timestep demonstrate improved multi-view consistency compared to the original edited latents, $\ze_t$.
% Since the entire image editing process is divided into multiple diffusion timesteps, the edited latent $\ze_t$ undergoes minimal changes from $\zs_t$ at each timestep and minor inconsistency across views.
The image editing process, segmented into multiple diffusion timesteps, ensures $\ze_t$ undergoes only minimal changes from $\zs_t$ and maintains minor inconsistency across views at each step.
% \textcolor{blue}{one sentence to describe it can be calibrated by 3DGS}
% \textcolor{blue}{Such incremental adjustments safeguard against mode collapse in $\gft$ during the fine-tuning phase.}
% The rapid training and rendering capabilities of 3DGS enables fine-tuning and rendering at each timestep.
Thus, by continuously calibrating the incoherent contents of $\ze_t$ using 3DGS, this mechanism effectively prevents the inconsistencies from accumulating, thereby avoiding divergence among the multi-view edited images.
In our ablation study, detailed in Sec.~\ref{}, we demonstrate the significant capability of this mechanism to address multi-view inconsistencies.


\subsection{Iterative Pattern Extension}
\label{sec:iter}
To further alleviate the multi-view inconsistency issue, we extend our VCEditor to an interative pattern.
Following the image-guided editing pipeline in Sec.~\ref{3dgs editing}, we define each sequence of transitions ---from $\gsrc$ to $\Isrc$, from $\Isrc$ to $\Iedt$, and from $\Iedt$ to $\gedt$---as an iteration.

Upon completion of one iteration, the edited 3DGS, $\gedt$, is continuously forwarded to the subsequents, serving as the new $\gsrc$.
This iterative pattern fosters a mutual cycle, where the $\Iedt$ and $\gedt$ progressively refines each other, leading to continuous improvement in consistency and quality.
Each iteration brings the 3DGS closer to the user's prompt, facilitating easier image editing in subsequent iterations.
This leads to more consistent and higher-quality image guidance, $\Iedt$, which in turn refines the 3DGS for an improved $\gedt$. \textcolor{blue}{[thanks to the consistency control mechnasiam, xxx]}
% Some views that are inconsistently edited in the first iteration get the chance to be better edited in the next iteration, leading to a high-quality image guidances, $\Iedt$, which in turn refines the 3DGS and achieves a better $\gedt$.
